Interactive Communication in Bilateral Trade

We define a model of interactive communication where two agents with private types can exchange information before a game is played. The model contains Bayesian persuasion as a special case of a one-round communication protocol. We define message complexity corresponding to the minimum number of interactive rounds necessary to achieve the best possible outcome. Our main result is that for bilateral trade, agents don't stop talking until they reach an efficient outcome: Either agents achieve an efficient allocation in finitely many rounds of communication; or the optimal communication protocol has infinite number of rounds. We show an important class of bilateral trade settings where efficient allocation is achievable with a small number of rounds of communication.

==> ex_non_voluntary.tex <==
\newpage
\section{An Example of Non-Voluntary Communication}
\textcolor{red}{Doesn't seem to work.}
Bob's private information is: a secret password $p$ and two secret bits $b_1$ and $b_2$, all of which are independent. $p$ is uniformly drawn from a large set. $b_1 = 1$ with probability $0.5$ and $0$ otherwise, and same for $b_2$.

Sally has two types $s_1$ and $s_2$ with equal probability. If her type is $s_1$, $b_1$ is her preferred bit and $b_2$ is her backup bit. If her type is $s_2$, $b_2$ is her preferred bit and $b_1$ is her backup bit.

\paragraph{The base game.}
\begin{itemize}
    \item Sally can choose to do nothing at the base game, giving $(u_S, u_B) = (0, 0)$.
    \item She can choose a bit to guess. If the bit is her preferred bit and she is correct: $(u_S, u_B) = (2, 1)$. If the bit is her backup bit and she is correct: $(u_S, u_B) = (1, 2)$. If she is wrong in guessing, $(u_S, u_B) = (-100, -100)$.
    \item She can guess the password and her preferred bit. If she is correct in both guesses: $(u_S, u_B) = (1000, -10000)$. If she is wrong in either guess, $(u_S, u_B) = (-100, -100)$.
\end{itemize}
 
\paragraph{At $t = 0$.}
Sally is not sure about Bob's secret bits, so she just does nothing to avoid huge penalty of guessing wrong, giving $(\pi_S^0, \pi_B^0) = (0, 0)$.

\paragraph{At $t = 1$.}
Bob can reveal his first secret bit $b_1$, which Sally will correctly guess. It gives $(\pi_S^1, \pi_B^1) = (1.5, 1.5)$. Bob cannot do better without knowing anything about Sally's type: Firstly there is no reason for him to reveal his password $p$. There is always at least at least half of Sally's guesses on her preferred bit -- If she guesses $b_2$ when her type is $s_1$, she must also guess $b_2$ when her type is $s_2$.

\paragraph{At $t = 2$.}
Sally's optimal strategy is to say nothing in this round. It gives $(\pi_S^2, \pi_B^2) = (1.5, 1.5)$. The optimality comes from $\pi_S^2 \geq \pi_S^1$ and $\pi_S^2 + \pi_B^2 \leq 3$.

\paragraph{At $t = 2$ but the password $p$ is common knowledge.}
Sally's optimal strategy is to reveal her type. \textcolor{red}{Doesn't seem to work.}

\paragraph{At $t = 3$.}
Bob can reveal his secret password $p$ in this round. $\pi_B^3 \geq 2$ and thus $\pi_S^3 \leq 3 - \pi_B^3 = 1 < \pi_S^2$.


